Pair Siegel-Veech constants for branched covers of tori and Veech surfaces

For a locus $\mathcal{E}$ of branched covers of tori satisfying a monodromy assumption, we show there exists an explicit constant $c_A(\mathcal{E})$ so that the number of pairs of saddle connections on surfaces in $\mathcal{E}$ of length at most $R$ and cross product at most $A$ grows like $c_A(\mathcal{E})R^2$ for every Diophantine surface in $\mathcal{E}$; this constant is moreover piecewise linear in $A$. In particular, this covers the case of billiards on rectangles with a barrier. Similar pointwise results are shown for Veech surfaces. The proof uses work of Margulis-Mohammadi on the quantitative inhomogeneous Oppenheim conjecture.

==> Figures/balanced-covers-command.tex <==
\newcommand{\BalancedCoversFigure}[1][1]{%
  \scalebox{#1}{%
    \begin{tikzpicture}[x=1pt,y=1pt,line width=.65pt,draw=black!92,line join=round,line cap=round]
    \path[use as bounding box] (0,0) rectangle (452,178);

    % (a) Three rectangles and their cyclic gluings.
    \filldraw[fill=gray!8] (55.20000,115.80000) rectangle (96.80000,149.40000);
    \draw (76.00000,126.20000) -- (76.00000,139.00000);
    \fill[black!92] (76.00000,126.20000) circle[radius=1.45pt];
    \fill[black!92] (76.00000,139.00000) circle[radius=1.45pt];
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (69.12000,129.60000) {$A$};
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (82.88000,129.60000) {$B$};
    \filldraw[fill=gray!8] (19.20000,53.40000) rectangle (60.80000,87.00000);
    \draw (40.00000,63.80000) -- (40.00000,76.60000);
    \fill[black!92] (40.00000,63.80000) circle[radius=1.45pt];
    \fill[black!92] (40.00000,76.60000) circle[radius=1.45pt];
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (33.12000,67.20000) {$B$};
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (46.88000,67.20000) {$C$};
    \filldraw[fill=gray!8] (91.20000,53.40000) rectangle (132.80000,87.00000);
    \draw (112.00000,63.80000) -- (112.00000,76.60000);
    \fill[black!92] (112.00000,63.80000) circle[radius=1.45pt];
    \fill[black!92] (112.00000,76.60000) circle[radius=1.45pt];
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (105.12000,67.20000) {$C$};
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (118.88000,67.20000) {$A$};
    \draw (32.00000,91.00000) arc[start angle=180,end angle=120,radius=44.0pt];
    \fill[black!92] (54.00000,129.10512) -- (49.78590,128.40416) -- (51.28590,125.80608) -- cycle;
    \draw (98.00000,129.10512) arc[start angle=60,end angle=0,radius=44.0pt];
    \fill[black!92] (120.00000,91.00000) -- (121.50000,95.00000) -- (118.50000,95.00000) -- cycle;
    \draw (98.00000,52.89488) arc[start angle=-60,end angle=-120,radius=44.0pt];
    \fill[black!92] (54.00000,52.89488) -- (56.71410,49.59584) -- (58.21410,52.19392) -- cycle;
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (76.00000,10.00000) {(a) $\kappa=(2,2)$};

    % (b) Two squares with paired slits.
    \filldraw[fill=gray!8] (166.00000,70.00000) rectangle (223.50000,127.50000);
    \draw (186.12500,117.15000) -- (175.77500,102.77500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (177.05464,110.66716) {$a$};
    \draw (180.95000,84.37500) -- (199.35000,84.37500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (190.15000,77.47500) {$b$};
    \draw (191.30000,99.32500) -- (214.30000,118.30000);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (205.85464,103.00991) {$c$};
    \fill[black!92] (186.12500,117.15000) circle[radius=1.45pt];
    \fill[black!92] (175.77500,102.77500) circle[radius=1.45pt];
    \fill[black!92] (180.95000,84.37500) circle[radius=1.45pt];
    \fill[black!92] (199.35000,84.37500) circle[radius=1.45pt];
    \fill[black!92] (191.30000,99.32500) circle[radius=1.45pt];
    \fill[black!92] (214.30000,118.30000) circle[radius=1.45pt];
    \filldraw[fill=gray!8] (231.55000,70.00000) rectangle (289.05000,127.50000);
    \draw (251.67500,117.15000) -- (241.32500,102.77500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (242.60464,110.66716) {$a$};
    \draw (246.50000,84.37500) -- (264.90000,84.37500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (255.70000,77.47500) {$b$};
    \draw (256.85000,99.32500) -- (279.85000,118.30000);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (271.40464,103.00991) {$c$};
    \fill[black!92] (251.67500,117.15000) circle[radius=1.45pt];
    \fill[black!92] (241.32500,102.77500) circle[radius=1.45pt];
    \fill[black!92] (246.50000,84.37500) circle[radius=1.45pt];
    \fill[black!92] (264.90000,84.37500) circle[radius=1.45pt];
    \fill[black!92] (256.85000,99.32500) circle[radius=1.45pt];
    \fill[black!92] (279.85000,118.30000) circle[radius=1.45pt];
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (227.50000,10.00000) {(b) $\kappa=(1,1,1,1,1,1)$};

    % (c) Four squares with paired slits.
    \filldraw[fill=gray!8] (317.00000,105.55000) rectangle (374.50000,163.05000);
    \draw (330.22500,142.92500) -- (361.85000,150.97500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (344.85344,149.50167) {$a$};
    \draw (330.22500,142.92500) -- (331.37500,121.07500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (335.59337,130.15228) {$d$};
    \draw (330.22500,142.92500) -- (362.42500,117.62500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (349.29054,131.94933) {$e$};
    \fill[black!92] (361.85000,150.97500) circle[radius=1.45pt];
    \fill[black!92] (330.22500,142.92500) circle[radius=1.45pt];
    \fill[black!92] (331.37500,121.07500) circle[radius=1.45pt];
    \fill[black!92] (362.42500,117.62500) circle[radius=1.45pt];
    \filldraw[fill=gray!8] (382.55000,105.55000) rectangle (440.05000,163.05000);
    \draw (395.77500,142.92500) -- (427.40000,150.97500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (410.40344,149.50167) {$a$};
    \draw (396.92500,121.07500) -- (427.40000,150.97500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (408.80086,137.35128) {$b$};
    \draw (427.40000,150.97500) -- (427.97500,117.62500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (432.48679,132.28275) {$c$};
    \fill[black!92] (427.40000,150.97500) circle[radius=1.45pt];
    \fill[black!92] (395.77500,142.92500) circle[radius=1.45pt];
    \fill[black!92] (396.92500,121.07500) circle[radius=1.45pt];
    \fill[black!92] (427.97500,117.62500) circle[radius=1.45pt];
    \filldraw[fill=gray!8] (317.00000,40.00000) rectangle (374.50000,97.50000);
    \draw (330.22500,77.37500) -- (331.37500,55.52500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (335.59337,64.60228) {$d$};
    \draw (331.37500,55.52500) -- (361.85000,85.42500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (343.25086,71.80128) {$b$};
    \draw (331.37500,55.52500) -- (362.42500,52.07500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (347.43007,56.47064) {$f$};
    \fill[black!92] (361.85000,85.42500) circle[radius=1.45pt];
    \fill[black!92] (330.22500,77.37500) circle[radius=1.45pt];
    \fill[black!92] (331.37500,55.52500) circle[radius=1.45pt];
    \fill[black!92] (362.42500,52.07500) circle[radius=1.45pt];
    \filldraw[fill=gray!8] (382.55000,40.00000) rectangle (440.05000,97.50000);
    \draw (395.77500,77.37500) -- (427.97500,52.07500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (414.84054,66.39933) {$e$};
    \draw (427.40000,85.42500) -- (427.97500,52.07500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (432.48679,66.73275) {$c$};
    \draw (396.92500,55.52500) -- (427.97500,52.07500);
    \node[font=\fontsize{8}{10}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (412.98007,56.47064) {$f$};
    \fill[black!92] (427.40000,85.42500) circle[radius=1.45pt];
    \fill[black!92] (395.77500,77.37500) circle[radius=1.45pt];
    \fill[black!92] (396.92500,55.52500) circle[radius=1.45pt];
    \fill[black!92] (427.97500,52.07500) circle[radius=1.45pt];
    \node[font=\fontsize{10}{12}\selectfont,text=black!92,inner sep=0pt,anchor=base] at (378.50000,10.00000) {(c) $\kappa=(3,3,3,3)$};
    \end{tikzpicture}%
  }%
}

==> Figures/billiard-unfolding-command.tex <==
\newcommand{\BilliardUnfoldingFigure}[1][1]{%
  \scalebox{#1}{%
    \begingroup%
    \definecolor{billiardInk}{HTML}{141414}%
    \definecolor{billiardFill}{HTML}{F5F5F5}%
    \definecolor{billiardRed}{HTML}{D52937}%
    \definecolor{billiardGuide}{HTML}{AAAAAA}%
    \begin{tikzpicture}[
      x=55.2bp, y=55.2bp,
      color=billiardInk,
      line cap=round, line join=round,
      panel/.style={draw=billiardInk, fill=billiardFill, line width=.64bp},
      barrier/.style={line width=.68bp},
      fold/.style={draw=billiardGuide, line width=.22bp,
        dash pattern=on 1.28bp off 1.28bp, line cap=butt},
      barrier extension/.style={fold, line width=.16bp,
        dash pattern=on .88bp off 1.04bp},
      trajectory/.style={color=billiardRed, line width=.80bp},
      direction/.style={
        postaction={decorate},
        decoration={markings, mark=at position ##1 with
          {\arrow{Triangle[length=2.30bp,width=2.10bp]}}}},
      transition/.style={line width=.48bp,
        -{Triangle[length=2.45bp,width=1.98bp]}},
      panel label/.style={anchor=base, inner sep=0pt,
        font=\fontsize{8.6bp}{10bp}\selectfont},
      pics/edge mark/.style={code={
        \fill[billiardInk] (0,0) -- (-1.70bp,.79bp)
          -- (-1.70bp,-.79bp) -- cycle;
      }},
    ]

    % Match the reference image's outer margins.
    \path[use as bounding box] (-.21739,-.61159) rectangle (7.60870,1.26087);

    % (a) The billiard. The panel height is the drawing unit.
    \filldraw[panel] (0,0) rectangle (2,1);
    \draw[barrier] (1,0) -- (1,.4);
    \fill (1,.4) circle[radius=.83bp];
    \draw[trajectory] (.2,.64) -- (1.4,1) -- (2,.82) -- (.2,.28);
    \path[trajectory,direction=.59] (.2,.64) -- (1.4,1);
    \path[trajectory,direction=.60] (2,.82) -- (.2,.28);
    \fill[billiardRed] (.2,.64) circle[radius=.80bp];
    \node[panel label] at (1,-.347) {(a)\enspace $P_\alpha$};

    \draw[transition] (2.203,.5) -- (2.414,.5);

    % (b) The four reflected copies and the unfolded trajectory.
    \begin{scope}[shift={(2.60870,0)}]
      \filldraw[panel] (0,0) rectangle (2,1);
      \draw[fold] (0,.5) -- (2,.5) (1,0) -- (1,1);
      \foreach \barrierX in {.5,1.5} {
        \draw[barrier extension] (\barrierX,.2) -- (\barrierX,.8);
        \draw[barrier] (\barrierX,0) -- (\barrierX,.2)
          (\barrierX,.8) -- (\barrierX,1);
        \foreach \tipY in {.2,.8} {
          \fill (\barrierX,\tipY) circle[radius=.83bp];
        }
      }
      \draw[trajectory,direction=.60] (.1,.32) -- (1.9,.86);
      \fill[billiardRed] (.1,.32) circle[radius=.80bp];
      \node[panel label] at (1,-.347) {(b)\enspace unfolding $P_\alpha$};
      \draw[transition] (2.203,.5) -- (2.414,.5);
    \end{scope}

    % (c) The square tori. One and two marks pair the slit banks crosswise.
    \foreach \torusX/\doubleBank in {5.17391/.51159,6.30435/.48841} {
      \begin{scope}[shift={(\torusX,0)}]
        \filldraw[panel] (0,0) rectangle (1,1);
        \foreach \edgeY in {0,1} {
          \pic at (.534,\edgeY) {edge mark};
        }
        \foreach \edgeX in {0,1} {
          \foreach \markY in {.477,.538} {
            \pic[rotate=90] at (\edgeX,\markY) {edge mark};
          }
        }

        \fill[white] (.48841,.2) rectangle (.51159,.8);
        \foreach \bankX in {.48841,.51159} {
          \draw[line width=.48bp] (\bankX,.2) -- (\bankX,.8);
          \pic[rotate=90] at (\bankX,.507) {edge mark};
        }
        \pic[rotate=90] at (\doubleBank,.573) {edge mark};
        \foreach \tipY in {.2,.8} {
          \fill (.5,\tipY) circle[radius=.83bp];
        }
      \end{scope}
    }

    % The trajectory crosses the first slit, wraps around the second torus,
    % then crosses back to the first torus. Each segment has slope 0.3.
    \begin{scope}[shift={(5.17391,0)}]
      \draw[trajectory,direction=.60] (.1,.32) -- (.48841,.43652);
      \draw[trajectory,direction=.58] (.51159,.74348) -- (.9,.86);
      \fill[billiardRed] (.1,.32) circle[radius=.80bp];
    \end{scope}
    \begin{scope}[shift={(6.30435,0)}]
      \draw[trajectory,direction=.60] (0,.59) -- (.48841,.73652);
      \draw[trajectory,direction=.60] (.51159,.44348) -- (1,.59);
    \end{scope}
    \node[panel label] at (6.23913,-.347)
      {(c)\enspace $\mathbb{T}^2\mathbin{\#_\alpha}\mathbb{T}^2$};

    \end{tikzpicture}%
    \endgroup%
  }%
}

==> Figures/double-pentagon-command.tex <==
\newcommand{\DoublePentagonFigure}[1][1]{%
  \scalebox{#1}{%
    \begin{tikzpicture}[
      scale=2, line join=round, line cap=round,
      edge identification/.style={
        decorate,
        decoration={markings, mark=at position .5 with {
          \foreach \arrowindex in {1,...,##1} {
            \pgfmathsetlengthmacro{\arrowoffset}{(\arrowindex-(##1+1)/2)*5pt}
            \begin{scope}[xshift=\arrowoffset]
              \draw[thick] (-2.1pt,2.6pt) -- (1.9pt,0pt) -- (-2.1pt,-2.6pt);
            \end{scope}
          }
        }}
      }
    ]
      % Two regular pentagons reflected across their common vertical side.
      \foreach \k in {0,...,4} {
        \coordinate (P\k) at
          ({-cos(36)+cos(-36+72*\k)},{sin(-36+72*\k)});
        \coordinate (Q\k) at
          ({ cos(36)-cos(-36+72*\k)},{sin(-36+72*\k)});
      }

      \fill[gray!8] (P0)--(P1)--(P2)--(P3)--(P4)--cycle;
      \fill[gray!8] (Q0)--(Q1)--(Q2)--(Q3)--(Q4)--cycle;

      % Outer boundary and shared side.
      \draw[thick] (P1)--(P2)--(P3)--(P4)--(P0);
      \draw[thick] (Q1)--(Q2)--(Q3)--(Q4)--(Q0);
      \draw[densely dashed, gray] (P0)--(P1);

      % Each pair of directed edges has the same displacement vector.
      \foreach \marks/\pfrom/\pto/\qfrom/\qto in {
        1/P1/P2/Q4/Q0,
        2/P2/P3/Q3/Q4,
        3/P3/P4/Q2/Q3,
        4/P4/P0/Q1/Q2%
      }{
        \path[edge identification=\marks] (\pfrom)--(\pto);
        \path[edge identification=\marks] (\qfrom)--(\qto);
      }

      \node at ({-cos(36)},0) {$P$};
      \node at ({ cos(36)},0) {$Q$};
    \end{tikzpicture}%
  }%
}

==> Figures/slit-tori-command.tex <==
\newcommand{\SlitToriFigure}[1][1]{%
  \scalebox{#1}{%
    \begin{tikzpicture}[
      x=1pt,y=1pt,line width=.65pt,draw=black!92,
      line join=round,line cap=round,
      every node/.style={font=\fontsize{12}{14}\selectfont,
        text=black!92,inner sep=0pt,draw=none}
    ]
      \path[use as bounding box,draw=none] (0,0) rectangle (186,107);

      % Square position, chevron centers, tick heights, and slit-bank signs.
      \foreach \panelx/\chevroncenters/\tickheights/\uppersign/\lowersign in {
        5/{38}/{38}/+/-,
        105/{35.5,40.5}/{36.25,39.75}/-/+
      }{
        \begin{scope}[shift={(\panelx,15.5)}]
          \filldraw[fill=gray!8] (0,0) rectangle (76,76);

          \foreach \side in {0,76} {
            \foreach \cx in \chevroncenters {
              \draw ({\cx-2.1},{\side+2.8}) -- ({\cx+1.9},\side)
                -- ({\cx-2.1},{\side-2.8});
            }
            \foreach \ty in \tickheights {
              \draw ({\side-2.8},\ty) -- ({\side+2.8},\ty);
            }
          }

          \draw (0,0) -- (21,27);
          \fill[black!92,draw=none] (0,0) circle[radius=1.65pt]
            (21,27) circle[radius=1.65pt];
          \node[anchor=base west] at (27,28) {$\xi$};
          \node at (7.5,21) {$\uppersign$};
          \node at (19.5,11.5) {$\lowersign$};
        \end{scope}
      }
    \end{tikzpicture}%
  }%
}
